Sharpness Minimization Algorithms Do Not Only Minimize Sharpness To Achieve Better Generalization

Despite extensive studies, the underlying reason as to why overparameterized neural networks can generalize remains elusive. Existing theory shows that common stochastic optimizers prefer flatter minimizers of the training loss, and thus a natural potential explanation is that flatness implies generalization. This work critically examines this explanation. Through theoretical and empirical investigation, we identify the following three scenarios for two-layer ReLU networks: (1) flatness provably implies generalization; (2) there exist non-generalizing flattest models and sharpness minimization algorithms fail to generalize, and (3) perhaps most surprisingly, there exist non-generalizing flattest models, but sharpness minimization algorithms still generalize. Our results suggest that the relationship between sharpness and generalization subtly depends on the data distributions and the model architectures and sharpness minimization algorithms do not only minimize sharpness to achieve better generalization. This calls for the search for other explanations for the generalization of over-parameterized neural networks.

==> related_works.tex <==
\section{Related Works}\label{sec:related_works}



\paragraph{Empirical study on sharpness and generalization.} The investigation into the link between sharpness and generalization has its roots in the work of \citet{hochreiter1997flat}. A direct relationship among learning rate, batch size, generalization error, and the sharpness of the loss landscape was noted by \citet{keskar2016large,jastrzkebski2017three}.  \citet{dinh2017sharp} show that one can easily construct networks with good generalization but with arbitrary large sharpness by reparametrization, which suggests a strict positive correlation between sharpness and generalization is theoretically impossible in networks admitting certain rescaling symmetry. \citet{jiang2019fantastic} conducted an extensive empirical investigation on a range of generalization metrics, and their findings revealed that measures grounded in sharpness exhibit the strongest correlation with generalization.

\paragraph{Sharpness minimization algorithms.}
